What if Neural Networks had SVDs?

Various Neural Networks employ time-consuming matrix operations like matrix inversion. Many such matrix operations are faster to compute given the Singular Value Decomposition (SVD). Previous work allows using the SVD in Neural Networks without computing it. In theory, the techniques can speed up matrix operations, however, in practice, they are not fast enough. We present an algorithm that is fast enough to speed up several matrix operations. The algorithm increases the degree of parallelism of an underlying matrix multiplication $H\cdot X$ where $H$ is an orthogonal matrix represented by a product of Householder matrices. Code is available at www.github.com/AlexanderMath/fasth .

==> sections/9_local_minima.tex <==
\subsection{Additional Local Minimum. }\label{sup:spurious} 
This subsection experimentally address a theoretical concern raised by \cite{cayley1}. 
To maintain the SVD we need to perform optimization over weights constrained to be orthogonal. 
Instead of performing constrained optimization, we reparameterize the weights by using Householder matrices. 
This reparameterization may introduce additional "spurious" local minima \cite{cayley1}. 
Since we use optimization algorithms like gradient descent that converge to a local minimum, introducing local minima might substantially decrease the quality of the local minimum our optimization algorithm converges to. 

It can be proved \cite{cayley1} that two alternative techniques does not introduce any local minimum. 
These techniques use either the matrix exponential or the Cayley map, which as demonstrated in \Cref{subsec:running_time} are slower than our algorithm. 
From this perspective, our algorithm is faster but might add local minimum that decrease performance. 
One might then ask if the gains in running time is worth the potential risk of local minimum. 

To investigate this trade-off, we train the same Neural Network three times, each time using a different parameterization: the matrix exponential, the Cayley map and the Householder decomposition. 
It is possible to initialize all networks with the same weight even though we use a different parameterization, see the Supplementary Material \ref{sup:spurious}. 
To make sure we did not favor the Householder decomposition, we used the Cayley initialization from \cite{matrixexp2}. 

The experiment was carried out for two Neural Network classifiers on MNIST \cite{mnist}, one of depth $2$ and one of depth $4$. 
The experiment was repeated $8$ times, each time with a different random seed for the Cayley weight initialization. 
Since our goal is to investigate whether the Householder decomposition gets caught in poor local minima, something that only depends on the training data, we report training loss instead of validation loss. 
To remove clutter we computed a moving average of loss before computing the mean loss over the $8$ repetitions, see \Cref{fig:loss_curves2,fig:loss_curves4}. 


\paragraph{Local Minima. }
In theory the approaches based on the matrix exponential and the Cayley map introduce no local minima. 
Potential differences in training loss then cannot theoretically be explained by the introduction of local minima. 
However, experimentally, we find a small difference between the training loss of the two parameterizations, we denote this difference $\delta$. 
For both Neural Networks of depth $2$ and $4$, the converged training loss for the Householder approach is no more than $\delta$ away from one of the two other approaches, and the loss is less than that attained by the Exponential approach. 
For these hyperpameters, we can then theoretically not explain the difference in loss by the introduction of local minima. 


\paragraph{Conclusion. }
One might be concerned that the Householder decomposition introduces local minima. 
In our experiments we found no evidence to support this concern. 


\paragraph{Caveats. }The experiments were performed on a single data set for two architectures. 
As with most machine learning experiments, changing architecture, dataset, optimizer, step-size, batch-size, etc, might change the results. 
We leave further investigation of this issue for future work. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{plots/minima_2.pdf}
    \caption{Comparison of loss curves for depth $2$ Neural Networks with different orthogonal reparameterizations. 
    The loss at convergence is so small that it is not possible to conclude the Householder approach introduce local minima. }
    \label{fig:loss_curves2}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{plots/minima_4.pdf}
    \caption{Comparison of loss curves for depth $4$ Neural Networks with different orthogonal reparameterizations. 
    The loss at convergence is so small that it is not possible to conclude the Householder approach introduce local minima. }
    \label{fig:loss_curves4}
\end{figure}


\paragraph{Local Minima}
The loss part of the experiment was repeated 8 times. Our server has 8 GPUs, and we started one experiment on each GPU. This was fine for the loss experiments. Unfortunately, when comparing times, this is a bit unfair to the cayley/exponential map, since both of them has larger CPU usage than the Householder approach. 
This did not affect the loss part of the experiment, but it does affect the timing of the experiment. 
The time part of our expermient was thus only run once. 

So ours increase from 0.001290s to 0.00138 time when running 4, while theres increase from 0.015 to 0.4. This means that we can parallelize the WY decomposition while when they construct the matrix they cant parallelize in any way. We see a similar thing for matrix exponential and cayley.


==> sections/mops.tex <==
\subsection{Matrix Operations}\label{sup:proof_matrix_operations}


\paragraph{Proof of \Cref{lemma:propertis}. }

We consider a square weight matrix since $4$ out of the $5$ operations we consider are undefined for rectangular matrices. 
The SVD of a real square matrix $W\in\R^{d\times d}$ is $W=U \Sigma V^T$ where $\Sigma\in\R^{d\times d}$ is a diagonal matrix with $\Sigma_{ii}\ge 0$ and $U,V\in\R^{d\times d}$ are orthogonal matrices, i.e., $U^T=U^{-1}$ and $V^T=V^{-1}$. 

Some of the matrix operations concern the special case where $W=W^T$. In this case, the SVD simplifies to $W=U\Sigma U^T$, however, the values of $\Sigma_{ii}$ can be negative. 

\Cref{lemma:propertis} states five well-known linear algebra results. 
Each result allows fast computation of a different matrix operation when the SVD is known. 
After the lemma, we describe how each matrix operation relates to Neural Networks. 
\begin{lemma}Let $W$ have a SVD $W=U \Sigma V^T$, it holds that \label{lemma:propertis}
\begin{enumerate}
    \item \textbf{Determinant. }$|\text{det}(W)| =\prod_{i=1}^d \Sigma_{ii}$. 
    \item \textbf{Inverse. }$ W^{-1} = V \Sigma^{-1} U^T $. 
    \item \textbf{Largest singular value. }$\max_{i=1}^d \Sigma_{ii}$. 
    \item \textbf{Matrix exponential. }If $W=W^T$ then $W=U\Sigma U^T$, 
    $$e^W := \sum_{k=0}^\infty \frac{1}{k!}W^k=U e^\Sigma U^T, $$
    where $e^\Sigma$ is diagonal and $(e^\Sigma)_{ii} = e^{\Sigma_{ii}}$. Similar is true when $W^T=-W$. 
    \item \textbf{Cayley map.} If $W=W^T$ then $W=U\Sigma U^T$,
    \begin{align*}
        C:&=(I-W)(I+W)^{-1}\\&= U(I-\Sigma)(I+\Sigma)^{-1}U^T.
    \end{align*}
    Similar is true when $W^T=-W$. 
\end{enumerate}
\end{lemma}
\begin{proof}See the Supplementary Material \ref{sup:proof_matrix_operations}. 
\end{proof}
We now show how each result in \Cref{lemma:propertis} relates to the computation of matrix operations in Neural Networks. 

Result 1 and 2 allow the computation of matrix determinant and matrix inversion in $O(d)$ time. 
Both operations are used by Normalizing Flows \cite{emerging}. 
Computing these operations with standard operations like \textsc{pytorch.inverse(..)} and  \textsc{pytorch.slogdet(..)} \cite{pytorch} take $O(d^3)$ time.
Previous work suggests using the PLU and QR decomposition to circumvent the $O(d^3)$ standard operations 
\cite{glow,emerging}. 
We discuss the advantages of the SVD approach in \Cref{sec:rw}. 

Result 3 allows the \emph{exact} computation of the largest singular value in $O(d)$ time. 
The largest singular value is used for Spectral Normalization \cite{sngan}. 
It is usually \emph{approximated} in $O(d^2r)$ time by running $r$ rounds of the power iteration algorithm.  
Similar speed-ups are possible when $W$ is rectangular. 

Result 4 and 5 allow the computation of the matrix exponential and the Cayley map in $O(d)$ time. 
Both operations are used by \cite{matrixexp2}, computed in $O(d^3)$ by 
Padé approximation and \textsc{pytorch.solve(..)}, respectively. 

See \Cref{tbl:overview} for a summary. 


\input{tables/tbl-operators.tex}


\paragraph{Remark.} All operations from \Cref{lemma:propertis} can be computed in $O(d)$ time, faster than computing a single matrix-vector multiplication $O(d^2)$. 
For example, if we compute $W^{-1}x$ for $x\in \R^{d}$ the time consumption is dominated by the multiplication and not the matrix inversion. 




\begin{proof}
(1) $|\text{det}(W)|=|\text{det}(U)|\cdot |\text{det}(\Sigma)|\cdot |\text{det}(V^T)|$ since the determinant of a product is equal to the product of determinants. 
But the determinant of orthogonal matrices $U$ and $V^T$ is $\pm 1$, so $|\text{det}(W)|=|\text{det}(\Sigma)|$. 
But $\Sigma$ is diagonal and all entries are positive so $|\text{det}(W)|=\text{det}(\Sigma)=\prod_{i=1}^d\Sigma_{ii}$. 

(2) Let us check that $W\cdot W^{-1}=I$. Recall that $V^T=V^{-1}$ and $U^T=U^{-1}$. 
\begin{align*}
W W^{-1} &= U\Sigma V^T V \Sigma^{-1} U^T \\
&= U \Sigma \Sigma^{-1} U^T \\
&= U U^T= I
\end{align*}

(3) The \emph{singular} values are defined to be the entries of $\Sigma$, the diagonal matrix of the \emph{Singular} Value Decomposition. 

(4) If $W$ is symmetric then $W=U\Sigma U^T$. Inserting this decomposition into the matrix exponential, we get 
\begin{align*}
e^{U\Sigma U^T}&=
\sum_{k=0}^\infty \frac{1}{k!} (U\Sigma U^T)^k 
\\&= 
\sum_{k=0}^\infty \frac{1}{k!} U \Sigma^k U^T
\\&=
U\left(\sum_{k=0}^\infty \frac{1}{k!}  \Sigma^k\right) U^T
\\&=
U e^\Sigma  U^T
\end{align*}
If $W$ is skew-symmetric, $W^T=-W$, we get $W=U\Sigma U^T$ but for complex $U$. 

(5) If $W$ is symmetric then $W=U\Sigma U^T$. Inserting this decomposition into the Cayley transform yields
\begin{align*}
C&=(I-W)(I+W)^{-1}\\
&=(U I U^T-U\Sigma U^T)(U I U^T - U\Sigma U^T)^{-1}\\
&= U(I-\Sigma)U^T U (I+\Sigma)^{-1} U^T\\
&=U(I-\Sigma)(I+\Sigma)^{-1}U^T. 
\end{align*} 
If $W$ is skew-symmetric, $W^T=-W$, we get $W=U\Sigma U^T$ but for complex $U$. 
\end{proof}

\paragraph{Weight Decay.} 
Weight decay is a regularizer that adds the Frobenious norm of a weight matrix to the loss function. 
The Frobenious norm is $||W||_F^2=\sum_{ij}W_{ij}^2=\sum_{i=1}^d \Sigma_{ii}^2$.
If the SVD is given the norm can be computed in $O(d)$ instead of $O(d^2)$. 

\paragraph{Compression with Truncated SVD. }
Neural Networks can be compressed by truncating the SVD of all weight matrices, see e.g. \cite{compresswithsvd}.  
This usually requires computing the SVD in $O(d^3)$ time.
If the SVD is given, we only need to compute the largest $k$ singular values and discard the remaining singular values/vectors. 
Computing the $k$ largest singular values could be done by sorting all singular values in $O(d \lg d)$ time. 
It is possible to get $O(d)$ time by using the selection algorithm to get the $k$'th largest singular value in $O(d)$ time, then partition around the $k$'th largest element. 


\paragraph{Pseudo-Inverse. }
The pseudo-inverse of a rectangular matrix $M\in \R^{m\times n}$ is usually computed by using the SVD to compute the reciprocal of the singular values. 
The time consumption is dominated by computing the SVD which, if $m>n$, takes $O(m^2n)$ time. 
If the SVD is given it takes $O(n)$ time to compute the reciprocal of the singular values.  

\paragraph{Condition Number. }The condition number of a square matrix is $\kappa = \max_{i}\Sigma_{ii}/\min_{i} \Sigma_{ii}$, normally computed by first computing the SVD in $O(d^3)$ time.  
If the SVD is already given it can be computed in $O(d)$ time. 


\clearpage 
